A Framework for Sample Efficient Interval Estimation with Control Variates

We consider the problem of estimating confidence intervals for the mean of a random variable, where the goal is to produce the smallest possible interval for a given number of samples. While minimax optimal algorithms are known for this problem in the general case, improved performance is possible under additional assumptions. In particular, we design an estimation algorithm to take advantage of side information in the form of a control variate, leveraging order statistics. Under certain conditions on the quality of the control variates, we show improved asymptotic efficiency compared to existing estimation algorithms. Empirically, we demonstrate superior performance on several real world surveying and estimation tasks where we use the output of regression models as the control variates.

==> application.tex <==
\section{Applications}
\subsection{Certifying Classification and Regression Performance}


From \corref{cor:bounded_example}, for $\epsilon \in [-1, 1]$, this means that with probability $> 1 - 2\zeta$,
$$
    \E[\epsilon] \in \left[
        \zeta^{1/m} \epsilon_{(1)} - (1 - \zeta^{1/m}),
        \zeta^{1/m} \epsilon_{(m)} + (1 - \zeta^{1/m})
    \right]
$$
Since we define $y = \hat{y} - \epsilon$, thus $\E[Y] = \frac{1}{n}\sum_{i=1}^n f(X_i) - \E[\epsilon]$, so
\begin{align*}
    \E[Y] \in \Bigg[
        & \frac{1}{n}\sum_{i=1}^n f(X_i) - \zeta^{1/m} \epsilon_{(m)} - (1 - \zeta^{1/m}), \\
        & \frac{1}{n}\sum_{i=1}^n f(X_i) - \zeta^{1/m} \epsilon_{(1)} + (1 - \zeta^{1/m}) \Bigg]
\end{align*}


\subsection{Semi-Supervised Mean Estimation} \label{sec:semisup_mean}
Consider two jointly-distributed random variables $X \in \Xc$ and $Y \in \R$ where we have $m$ labeled pairs $\{(x_i, y_i)\}_{i=1}^m$ and $n \gg m$ additional unlabeled examples $\{x'_i\}_{i=1}^n$. Let $f: \Xc \to \R$ be an arbitrary regression model, and define $\tY = f(X)$ to be the control variate for $Y$. By the Law of Large Numbers, $\frac{1}{n} \sum_{i=1}^n f(x'_i)$ is a very accurate estimate of $\E[\tY]$ for large $n$. We now have the setup described in Section~\ref{sec:control_variates}: $m$ samples $\{(y_i, \ty_i)\}_{i=1}^m$ along with a known value for $\E[\tY]$. We can calculate confidence intervals for $\E[Y]$ using our method of order statistics.

\subsection{Semi-Supervised Covariance Estimation}
In addition to setting described previously in Section~\ref{sec:semisup_mean}, we can additionally consider the case where we have a third random variable $W \in \R$, and suppose that we have a sample of $W$ corresponding to each sample of $X$. Our goal is to learn the covariance between $Y$ and $W$.

We can pose this estimation problem as a mean estimation task as follows. Defining $Z = YW - Y \E[W] = Y(W - \E[W])$, we have
\begin{align*}
    \Cov[Y, W]
    &= \E[YW] - \E[Y]\E[W] \\
    &= \E\left[YW - Y \E[W]\right]
     = \E[Z]
\end{align*}

Letting $\hat{Z} = f(X) (W - \E[W])$ and letting $\epsilon = \hat{Z} - Z$, we can directly apply the mean estimation technique for getting a confidence interval for the covariance, $\E[Z]$.

==> old.tex <==



\begin{proof}[Proof of Lemma~\ref{lemma:order_bound}]
Let $B_i$ be the event $X_i > \E[X] - c$. We first need to who a lower bound to $\Pr[B]$ in the following Lemma.
\begin{lemma}
\label{lemma:single}
Let $X$ be a bounded random variable in $[a, b]$. Then, $\forall c \in [0, b-a]$,
 $$
    P(X > \E[X] - c) \geq \frac{c}{b - \E[X] + c}.
$$
\end{lemma}

For some $c \in (0, b-a)$. Then,
% \begin{align*}
%     \Pr(X_{(m)} \leq \E[X] - c)
%     &= \prod_{i=1}^m \left(1 - P(B_i)\right) \\
%     &\leq \left(1 - \frac{c}{b - \E[X] + c}\right)^m
% \end{align*}
% % Because the RHS is monotonically decreasing with $\E [X]$, then 
% % \begin{align*}
% %     \Pr[\E[X] \geq X_{(m)}+c] \leq \left(1 - \frac{c}{b - X_{(m)}}\right)^m
% % \end{align*}
% 
% \begin{align*}
%     c
%     &= (1 - \zeta^{1/m})(b - \E[X] + c) \\
%     &= \zeta^{-1/m}(1 - \zeta^{1/m})(b - \E[X]) \\
%     &= (\zeta^{-1/m} - 1)(b - \E[X])
% \end{align*}
%Similarly we have 
\begin{align*}
    &\Pr[X_{(m-k)} \leq \Eb[X] - c] \\
    &= \sum_{i=0}^k \binom{m}{i} \Pr[B]^i (1 - \Pr[B])^{m-i} \numberthis\label{eq:order_stats} \\
    &\leq \sum_{i=0}^k \binom{m}{i} (1 - \Pr[B])^{m-i} \\
    &\leq \left( \sum_{i=0}^k \binom{m}{i} \right) (1 - \Pr[B])^{m-k} \\
    &\leq (1+m)^k \left(1 - \frac{c}{b - \E[X] + c}\right)^{m-k} 
\end{align*}
(Missing a 1+m here, to fix later). 
Setting the RHS $\leq \zeta$ and we get
\begin{align*}
   &k \log m + (m-k)\log \left(1 - \frac{c}{b - \E[X] + c}\right) \leq \log \zeta 
\end{align*}
Which is equivalent to
\begin{align*}
   & \frac{c}{b - \E[X] + c} \geq 1 - \stuffn
\end{align*}
Solving for $c$ we get
\begin{align*}
    c
    &= \left(1 - \stuffn\right)(b - \E[X] + c) \\
    &= \stuff\left(1 - \stuffn\right)(b - \E[X]) \\
    &= \left(\stuff - 1\right)(b - \E[X])
\end{align*}
Then
\begin{align*}
    \E[X] - c
    &= \E[X] - \left(\stuff - 1\right)(b - \E[X]) \\
    &= b - \stuff(b - \E[X])
\end{align*}
so
$$
     \Pr\left(X_{(m)} \leq b - \stuff(b - \E[X])\right) \leq \zeta.
$$
By symmetry, we can prove the other direction
$
    P\left(X_{(1)} \geq a + \zeta^{-1/m}(\E[X] - a)\right) \leq \zeta
$.

What remains to prove is Lemma~\ref{lemma:single}. We will now prove it. 

\begin{proof}[Proof of Lemma~\ref{lemma:single}]
Note that since $b - \E[X] \geq 0$ and $c \geq 0$, we have $b - \E[X] + c \geq c$, so the RHS is always $\leq 1$.

For simplicity, assume that $X$ is bounded in $[0, 1]$. Later in the proof, we show the general case.

First, consider the trivial case where $c > \E[X]$. Then the statements are clearly true:
$$
    \Pr(X > \E[X] - c) = 1 > \frac{c}{1 - \E[X] + c}.
$$
Now, consider the case where $c \in [0, \E[X]]$. Define $\delta_c \equiv P(B_c)$ where $B_c$ is the event $X > \E[X] - c$. Thus,
\begin{align*}
    \E[X]
    &= \E[X|B_c] \Pr(B_c) + \E[X|\bar{B_c}] \Pr(\bar{B_c}) \\
    &= \E[X|B_c] \delta_c + \E[X|\bar{B_c}] (1 - \delta_c) \\
    &\leq 1 \cdot \delta_c + (\E[X] - c) (1 - \delta_c) \\
    &= (1 - \E[X] + c) \delta_c + \E[X] - c.
\end{align*}
Solving for $\delta_c$ yields $\delta_c \geq \frac{c}{1 - \E[X] + c}$, as desired.

% If we instead considered the event $X \geq \E[X]-c$, then $\E[X|\bar{B_c}] < \E[X]-c$ (strict inequality), in which case $\delta_c > \frac{c}{1 - \E[X] + c}$, also as desired.

Now, we consider the general case where $X$ is a bounded r.v. in $[a, b]$. Define $Y = \frac{1}{b-a}(X-a)$, which is a r.v. bounded in $[0, 1]$. Applying the result above, we have for all $z \in [0, 1]$,
\begin{align*}
    &\Pr(Y > \E[Y] - z) \\
    &= \Pr\left(\frac{1}{b-a}(X-a) > \frac{1}{b-a}\E[X-a] - z\right) \\
    &= \Pr(X > \E[X] - z(b-a)) \\
    &\geq \frac{z}{1 - \E[Y] + z} 
    = \frac{z}{1 - \frac{1}{b-a}\E[X-a] + z} \\
    &= \frac{z(b-a)}{b - \E[X] + z(b-a)}
\end{align*}
Substituting $c = z(b-a)$ so that $c \in [0, b-a]$ yields the desired result, $P(X > \E[X] - c) = \frac{c}{b - \E[X] + c}$. 
\end{proof}\end{proof}


Consider a true distribution $P^*(X, Y)$ over random variables $X \in \Xc$ and $Y\in \mathcal{Y} \subseteq R^d$. We would like to estimate some property $\theta$ about $Y$, that is, we have an unbiased estimation function $A: (\Xc \times \mathcal{Y}) \to \R^k$. We assume the estimator is exchangeable: for any permutation function $\sigma$ we have $A(x_{1:m}, y_{1:m}) = A(\sigma(x_{1:m}), \sigma(y_{1:m}))$. Furthermore, we assume that the variance of the estimator is $\propto 1/m$.

For example, this is asymptotically true of the MLE estimator, which converges in distribution to $\mathcal{N}(\theta, I(\theta)^{-1}/m)$ as $m \to \infty$.

We assume that we can sample $X$ efficiently, but we have a limited budget of sampling $m$ examples from $P(Y|X)$. We compare the mean squared error of our estimate of $\theta$ under two options:
\begin{enumerate}
    \item Sample $\{ (x_i, y_i) \}_{i=1}^m$ and use the estimator directly $A(x_{1:m}, y_{1:m})$.

    Since the estimator is unbiased, the mean squared error of the estimator only depends on its variance. Therefore, this option has error $\propto \frac{1}{m}$.

    \item We are given a classifier $f: \Xc \to \mathcal{Y}$ with unknown performance. We sample $\{ (x_i, y_i) \}_{i=1}^m$ to validate its performance. We are also given a (practically infinite) set $\{ x_i \}_{i=1}^n$, where $n \gg m$, and then compute $\hy_i = f(x_i)$. We estimate $\theta$ with $A(x_{1:n}, \hy_{1:n})$.

    Suppose that for each $x_i$, the true label is $y_i = \E_{Y|X=x_i}[Y]$. Let $\epsilon_i$ denote the error from $f(x_i)$, so $\hy_i = y_i + \epsilon_i$.
\end{enumerate}

The question is whether we can obtain lower error with option 2.

We start by giving a bound on the probability that the deviation of a random variable $X$ from its mean is too large. Notably, this bound is better than what can be obtained by Hoeffding's inequality. For any random variable $X$ bounded in $[a, b]$:
\begin{align}
    \forall c \geq 0.\
    \Pr\left( X > \E[X] - c \right)
    &\geq \min\left\{\frac{c}{b-a}, 1\right\} \tag{Ours} \\
    &\geq 1 - e^{-2 c^2 / (b-a)^2} \tag{Hoeffding}
\end{align}

\begin{lemma}
Let $X$ be a bounded random variable in $[a, b]$. Then, $\forall c \in [0, b-a]$,
 $$
    P(X > \E[X] - c) \geq \frac{c}{b - \E[X] + c}
    \qquad\text{and}\qquad
    P(X \geq \E[X] - c) > \frac{c}{b - \E[X] + c}.
$$
\end{lemma}
\begin{proof}
Note that since $b - \E[X] \geq 0$ and $c \geq 0$, we have $b - \E[X] + c \geq c$, so the RHS is always $\leq 1$.

For simplicity, assume that $X$ is bounded in $[0, 1]$. Later in the proof, we show the general case.

First, consider the trivial case where $c > \E[X]$. Then the statements are clearly true:
$$
    P(X > \E[X] - c) = P(X \geq \E[X] - c) = 1 > \frac{c}{1 - \E[X] + c}.
$$
Now, consider the case where $c \in [0, \E[X]]$. Define $\delta_c \equiv P(B_c)$ where $B_c$ is the event $X > \E[X] - c$. Thus,
\begin{align*}
    \E[X]
    &= \E[X|B_c] \Pr(B_c) + \E[X|\bar{B_c}] \Pr(\bar{B_c}) \\
    &= \E[X|B_c] \delta_c + \E[X|\bar{B_c}] (1 - \delta_c) \\
    &\leq 1 \cdot \delta_c + (\E[X] - c) (1 - \delta_c)
     = (1 - \E[X] + c) \delta_c + \E[X] - c.
\end{align*}
Solving for $\delta_c$ yields $\delta_c \geq \frac{c}{1 - \E[X] + c}$, as desired.

If we instead considered the event $X \geq \E[X]-c$, then $\E[X|\bar{B_c}] < \E[X]-c$ (strict inequality), in which case $\delta_c > \frac{c}{1 - \E[X] + c}$, also as desired.

Now, we consider the general case where $X$ is a bounded r.v. in $[a, b]$. Define $Y = \frac{1}{b-a}(X-a)$, which is a r.v. bounded in $[0, 1]$. Applying the result above, we have for all $z \in [0, 1]$,
\begin{align*}
    P(Y > \E[Y] - z)
    &= P\left(\frac{1}{b-a}(X-a) > \frac{1}{b-a}\E[X-a] - z\right)
    = P(X > \E[X] - z(b-a)) \\
    &\geq \frac{z}{1 - \E[Y] + z}
    = \frac{z}{1 - \frac{1}{b-a}\E[X-a] + z}
    = \frac{z(b-a)}{b - \E[X] + z(b-a)}.
\end{align*}
Substituting $c = z(b-a)$ so that $c \in [0, b-a]$ yields the desired result, $P(X > \E[X] - c) = \frac{c}{b - \E[X] + c}$. The derivation for $P(X \geq \E[X]-c)$ is essentially identical.
\end{proof}

\begin{lemma}
Let $X_1, \dotsc, X_m$ be independent samples of a random variable $X$ bounded in $[a, b]$. Let $X_{(i)}$ denote the $i$-th order statistic, so $X_{(1)} = \min_i X_i$ and $X_{(m)} = \max_i X_i$. Then $\forall z \in [0, 1]$,
$$
    P\left(X_{(1)} \geq a + \zeta^{-1/m}(\E[X] - a)\right) \leq \zeta
    \qquad\text{and}\qquad
    P\left(X_{(m)} \leq b - \zeta^{-1/m}(b - \E[X])\right) \leq \zeta.
$$
\end{lemma}
\begin{proof}
Let $B_i$ be the event $X_i > \E[X] - c$, for some $c \in [0, b-a$. Then,
$$
    P(X_{(m)} \leq \E[X] - c)
    = \prod_{i=1}^m \left(1 - P(B_i)\right)
    \leq \left(1 - \frac{c}{b - \E[X] + c}\right)^m.
$$
% Because the RHS is monotonically decreasing with $\E [X]$, then 
% \begin{align*}
%     \Pr[\E[X] \geq X_{(m)}+c] \leq \left(1 - \frac{c}{b - X_{(m)}}\right)^m
% \end{align*}
Setting the RHS equal to $\zeta$ and solving for $c$ yields
$$
    c
    = (1 - \zeta^{1/m})(b - \E[X] + c)
    = \zeta^{-1/m}(1 - \zeta^{1/m})(b - \E[X])
    = (\zeta^{-1/m} - 1)(b - \E[X]).
$$
Then,
$$
    \E[X] - c
    = \E[X] - (\zeta^{-1/m} - 1)(b - \E[X])
    = b - \zeta^{-1/m}(b - \E[X])
$$
so
$$
     P\left(X_{(m)} \leq b - \zeta^{-1/m}(b - \E[X])\right) \leq \zeta.
$$
By symmetry, we can prove the other direction
$
    P\left(X_{(1)} \geq a + \zeta^{-1/m}(\E[X] - a)\right) \leq \zeta
$.
\end{proof}

Re-arranging the lemma above yields
$$
    P\left(\E[X] \leq \zeta^{1/m} X_{(1)} + (1 - \zeta^{1/m})a \right) \leq \zeta
    \quad\text{and}\quad
    P\left(\E[X] \geq \zeta^{1/m} X_{(m)} + (1 - \zeta^{1/m})b \right) \leq \zeta.
$$
Thus, for $\epsilon \in [-1, 1]$, this means that with probability $> 1 - 2\zeta$,
$$
\E[\epsilon] \in \left[
    \zeta^{1/m} \epsilon_{(1)} - (1 - \zeta^{1/m}) ,\
    \zeta^{1/m} \epsilon_{(m)} + (1 - \zeta^{1/m})
\right].
$$
Since we define $y = \hat{y} - \epsilon$, thus $\E[Y] = \frac{1}{n}\sum_{i=1}^n f(X_i) - \E[\epsilon]$, so
$$
    \E[Y] \in \left[
        \frac{1}{n}\sum_{i=1}^n f(X_i) - \zeta^{1/m} \epsilon_{(m)} - (1 - \zeta^{1/m}), \
        \frac{1}{n}\sum_{i=1}^n f(X_i) - \zeta^{1/m} \epsilon_{(1)} + (1 - \zeta^{1/m})
    \right].
$$
Compare this with what we had before:
$$
    \E[Y] \in \left[
        \frac{1}{n} \sum_{i=1}^n f(X_i) - \epsilon_{(m)} - 2(1-\zeta^{1/m}), \
        \frac{1}{n} \sum_{i=1}^n f(X_i) - \epsilon_{(1)} + 2(1-\zeta^{1/m})
    \right].
$$


\begin{lemma}\label{lemma:delta}
Let $X$ be a bounded random variable in $[0, 1]$. Then,
$$
    \forall c \in [0, 1].\ \Pr(X > \E[X] - c) \geq c
    \qquad\text{and}\qquad
    \forall c \in [0, 1).\ \Pr(X \geq \E[X] - c) > c.
$$
The first inequality is sharp, \emph{i.e.} there exists a probability distribution over $X$ such that $\Pr(X > \E[X] - c) = c$.

By symmetry,
$$
    \forall c \in [0, 1].\ \Pr(X < \E[X] + c) \geq c
    \qquad\text{and}\qquad
    \forall c \in [0, 1).\ \Pr(X \leq \E[X] + c) > c.
$$
\end{lemma}
\begin{proof}
For any $c > \E[X]$, the statements are clearly true:
$$
    \Pr(X > \E[X] - c) = 1 \geq c
    \qquad\text{and}\qquad
    \Pr(X \geq \E[X] - c) = 1 > c.
$$

Now, consider a fixed $c \in [0, \E[X]]$. For arbitrary $\mu \in [c, 1]$, define $B_\mu$ as the event $X > \mu - c$, and define $\delta_\mu \equiv P(B_\mu)$. Let $\delta \equiv \delta_{\mu = \E[X]} = \Pr(X > \E[X] - c)$.

Similarly, define $B'_\mu$ as the event $X \geq \mu - c$, and define $\delta'_\mu$ and $\delta'$ accordingly. Then,
\begin{align*}
    0
    &\quad\leq\quad \E[X | \bar{B_\mu}]
    \quad\leq\quad \mu - c
    \quad<\quad \E[X | B_\mu]
    \quad\leq\quad 1 \\
    0
    &\quad\leq\quad \E[X | \bar{B'_\mu}]
    \quad<\quad \mu - c
    \quad\leq\quad \E[X | B'_\mu]
    \quad\leq\quad 1.
\end{align*}

Therefore,
\begin{align*}
    \E[X]
    &= \E[X|B_\mu] \Pr(B_\mu) + \E[X|\bar{B_\mu}] \Pr(\bar{B_\mu}) \\
    &= \E[X|B_\mu] \delta_\mu + \E[X|\bar{B_\mu}] (1 - \delta_\mu) \\
    &\leq \delta_\mu + (\mu - c) (1 - \delta_\mu)
     \leq \delta_\mu + \mu - c.
\end{align*}
\sj{I think it is better to not make the approximation and change this to
\[ \delta_\mu \geq \frac{c}{1-\mu+c} \]
}
and similarly,
\begin{align*}
    \E[X]
    &= \E[X|B'_\mu] \delta'_\mu + \E[X|\bar{B'_\mu}] (1 - \delta'_\mu) \\
    &< \delta'_\mu + (\mu - c) (1 - \delta'_\mu)
     \leq \delta'_\mu + \mu - c.
\end{align*}

Re-arranging the inequalities yields
$$
    \delta_\mu \geq \E[X] - \mu + c
    \qquad\text{and}\qquad
    \delta'_\mu > \E[X] - \mu + c.
$$

Since $c \leq \E[X]$ and the inequalities above hold for any choice of $\mu \in [c, 1]$, they must hold for $\mu = \E[X]$. This yields
$$
    \delta \geq c
    \qquad\text{and}\qquad
    \delta' > c,
$$
which concludes the proof, since $\delta = \Pr(X > \E[X]-c)$ and $\delta' = \Pr(X \geq \E[X]-c)$.

To show that $\Pr(X > \E[X] - c) \geq c$ is a tight inequality, consider $X \sim \mathsf{Bernoulli}(k)$ so $\E[X] = k$. At $c = k$, the inequality is tight: $\Pr(X > \E[X] - c) = \Pr(X > 0) = c$.
\end{proof}

It is easy to extend \lemref{lemma:delta} to a random variable bounded in an arbitrary interval $[a, b]$.

\begin{corollary}\label{cor:arbitrary_range}
Let $X$ be a bounded random variable in $[a, b]$. Then,
$$
    \forall c \in [0, b-a].\ \Pr(X > \E[X] - c) \geq \frac{c}{b-a}
    \quad\text{and}\quad
    \forall c \in [0, b-a).\ \Pr(X \geq \E[X] - c) > \frac{c}{b-a}.
$$
\end{corollary}
\begin{proof}
Define $Y = \frac{1}{b-a} (X-a)$, so now $Y$ is a random variable bounded in $[0, 1]$. Applying \lemref{lemma:delta} yields
\begin{align*}
    \Pr(Y > \E[Y] - z)
    &= \Pr\left(\frac{1}{b-a} (X-a) > \frac{1}{b-a} \E[X - a] - z \right) \\
    &= \Pr(X-a > \E[X-a] - z(b-a)) \\
    &= \Pr(X > \E[X] - z(b-a)) \\
    &\geq z.
\end{align*}
Substituting $c = z(b-a)$ gives the desired result.
\end{proof}

\begin{lemma}\label{lemma:max}
Let $X_1, \dotsc, X_m$ be independent samples of a random variable $X$ bounded in $[a, b]$. Let $X_{(i)}$ denote the $i$-th order statistic, so $X_{(1)} = \min_i X_i$ and $X_{(m)} = \max_i X_i$. Then,
\begin{gather*}
    \forall c \in [0, b-a].\
    \Pr\left( X_{(m)} \leq \E[X] - c \right) \leq \left( 1 - \frac{c}{b-a} \right)^m \\
    \forall c \in [0, b-a). \
    \Pr\left( X_{(m)} < \E[X] - c \right) < \left( 1 - \frac{c}{b-a} \right)^m.
\end{gather*}
The bound is tight if and only if $\Pr(X > \E[X] - c) = c/(b-a)$. Equivalently,
\begin{gather*}
    \forall \zeta \in [0, 1].\
    \Pr\left( X_{(m)} \leq \E[X] - (b-a) \left( 1 - \zeta^\frac{1}{m} \right) \right) \leq \zeta \\
    \forall \zeta \in (0, 1].\
    \Pr\left( X_{(m)} < \E[X] - (b-a) \left( 1 - \zeta^\frac{1}{m} \right) \right) < \zeta.
\end{gather*}
By symmetry,
\begin{gather*}
    \forall c \in [0, b-a].\
    \Pr\left( X_{(1)} \geq \E[X] + c \right) \leq \left( 1 - \frac{c}{b-a} \right)^m \\
    \forall c \in [0, b-a). \
    \Pr\left( X_{(1)} > \E[X] + c \right) < \left( 1 - \frac{c}{b-a} \right)^m \\
    \forall \zeta \in [0, 1].\
    \Pr\left( X_{(1)} \geq \E[X] + (b-a) \left( 1 - \zeta^\frac{1}{m} \right) \right) \leq \zeta \\
    \forall \zeta \in (0, 1].\
    \Pr\left( X_{(1)} > \E[X] + (b-a) \left( 1 - \zeta^\frac{1}{m} \right) \right) < \zeta.
\end{gather*}
\end{lemma}
\begin{proof}
Consider a fixed $c \in [0, b-a]$. Define $B$ as the event $X \geq \E[X] - c$, so by Lemma 1, $\Pr(B) \geq c/(b-a)$. 
$$
    \Pr\left( X_{(m)} \leq \E[X] - c \right)
    = \Pr(\bar B)^m
    = (1 - \Pr(B))^m
    \leq (1 - c/(b-a))^m
    = \zeta
$$
Similarly, if we define $B'$ as the event $X > \E[X] - c$, we have $\Pr(B') > c/(b-a)$.
$$    
    \Pr\left( X_{(m)} < \E[X] - c \right)
    = \Pr(\bar{B'})^m
    = (1 - \Pr(B'))^m
    < (1 - c/(b-a))^m
    = \zeta
$$
In both cases, solving for $c$ yields $c = (b - a) (1 - \zeta^{1/m})$.
\end{proof}

\begin{corollary}\label{corollary:max}
Let $X_1, \dotsc, X_m$ be independent samples of a random variable $X$ bounded in $[0, 1]$. Let $X_{(i)}$ denote the $i$-th order statistic, so $X_{(m)} = \max_i X_i$. Then,
\begin{gather*}
    \forall c \in [0, 1].\
    \Pr\left( X_{(m)} \leq \E[X] - c \right) \leq e^{-cm} \\
    \forall c \in [0, 1). \
    \Pr\left( X_{(m)} < \E[X] - c \right) < e^{-cm}.
\end{gather*}
The bound is tight if and only if $\Pr(X > \E[X] - c) = c = 0$. Equivalently,
\begin{gather*}
    \forall \zeta \in [0, 1].\
    \Pr\left( X_{(m)} \leq \E[X] + \frac{\ln z}{m} \right) \leq \zeta
    \\
    \forall \zeta \in (0, 1].\
    \Pr\left( X_{(m)} < \E[X] + \frac{\ln z}{m} \right) < \zeta.
\end{gather*}
As a special case, for $c \in [\E[X], 1)$ or equivalently $\zeta \in (0, e^{-m}]$, both probabilities are 0.
\end{corollary}
\begin{proof}
Combining \lemref{lemma:max} with the fact $\forall x \in \R.\ (1-x) \leq e^{-x}$, which is an equality if and only if $x = 0$, we have
\begin{gather*}
\forall c \in [0, 1].\ \Pr(X_{(m)} \leq \E[X] - c) \leq (1-c)^m \leq e^{-cm} \\
\forall c \in [0, 1).\ \Pr(X_{(m)} < \E[X] - c) < (1-c)^m \leq e^{-cm}
\end{gather*}
The right-most inequalities are equalities iff $c=0$. Setting $\zeta = e^{-cm}$ and solving for $c$ yields $c = -(\ln z)/m$, as desired.
\end{proof}

\begin{lemma}\label{lemma:mean}
Let $X_1, \dotsc, X_m$ be independent samples of a random variable $X$ bounded in $[a, b]$. Let $\bar{X} = \frac{1}{m} \sum_{i=1}^m X_i$ denote their mean. Hoeffding's one-sided inequality yields
$$
    \forall c \geq 0.\ \Pr(\bar{X} \leq \E[X] - c) \leq \exp\left[ -2m c^2 / (b-a)^2 \right].
$$
Setting $\zeta = \exp\left[ -2m c^2 / (b-a)^2 \right]$ and solving for $c$ yields $c = (b-a) \sqrt{-\frac{\ln\zeta}{2m}}$. Thus, equivalently,
$$
    \forall \zeta \in (0, 1].\
    \Pr\left( \bar{X} \leq \E[X] - (b-a) \sqrt{-\frac{\ln\zeta}{2m}} \right)
    \leq \zeta.
$$
\end{lemma}



% \textbf{Special Case: Mean Estimation}
% \begin{theorem}
% Option 2 is always worse!
% \end{theorem}

\subsection{Special Case: Weighted Average}
Suppose $Y \in [0, 1]$ with $\E[Y] = \mu$ and $\Cov[Y] = \Sigma \in \R^{d \times d}$. We start by considering a particular property $\theta = \E[\tA Y] = \tA \E[Y] = \tA \mu$ for some arbitrary given matrix $\tA \in \R^{k \times d}$. This setting represents a weighted average of $Y$. For example:
\begin{itemize}
    \item If $\tA = I_d$, then $\theta = \E[Y] = \mu$ is the element-wise average of $Y$.
    \item If $\tA = \mathbf{1}_d^T$, then $\theta = \E[\mathbf{1}_d^T Y] = \mathbf{1}_d^T \mu$ is the average sum of $Y$.
    \item If $\tA = (W^T W)^{-1} W^T$ for some fixed matrix $W \in \R^{d \times k}$, then $\theta = (W^T W)^{-1} W^T \mu$ minimizes $\|W \theta - Y\|_2$.
\end{itemize} 

From Section \ref{sec:linear_case}, we know that our unbiased estimator is
$$
    A(y_{1:l}) = \frac{1}{l} \sum_i \tA y_i.
$$

By the Real Spectral Theorem, since $\tA^T \tA$ is a real symmetric matrix, it is diagonalizable with respect to an orthonormal basis of its eigenvectors. Concretely, there exists a set of orthonormal eigenvectors $q_1, \dotsc, q_d$ with corresponding eigenvalues $\lambda_1, \dotsc, \lambda_d$ such that $\tA^T \tA = Q \Lambda Q^T \in \R^{d \times d}$, where $Q = [q_1, \dotsc, q_d]$ and $\Lambda = \diag(\lambda_1, \dotsc, \lambda_d)$. $Q$ is an orthogonal matrix. Furthermore, $\tA^T \tA$ is positive semi-definite, so all of the eigenvalues are non-negative: $\lambda_i \geq 0$.

\paragraph{Option 1.}
We draw $m$ independent examples $(x_i, y_i)$.
$$
    \Cov[A(y_{1:m})] = \frac{1}{m} \tA \Sigma \tA^T
$$
Since the bias of our estimator is 0, the MSE of our estimator is
\begin{align*}
    \E[\| A(y_{1:m}) - \tA \mu \|_2^2]
    &= \tr \Cov[A(y_{1:m})]
     = \frac{\tr(\tA\Sigma \tA^T)}{m}
     = \frac{\tr(\Sigma \tA^T\tA)}{m} \\
    &= \frac{\tr(\Sigma Q \Lambda Q^T)}{m}
     = \frac{1}{m} \sum_{i=1}^d \lambda_i q_i^T \Sigma q_i
\end{align*}

\paragraph{Option 2.}
We sample $n \gg m$ examples of $x_i$, then compute $\hy_i = f(x_i)$. Suppose that for each $x_i$, the true label is $y_i = \E_{Y|X=x_i}[Y]$. Let $\epsilon_i$ denote the error from $f(x_i)$, so $\hy_i = y_i + \epsilon_i$. Then
$$
    A(\hy_{1:n}) = \frac{1}{n} \sum_i \tA y_i +  \tA \epsilon_i
    % &\approx \mathcal{N}(A(g^*(x_1), \cdots, g^*(x_n)), \Gamma)
$$
The bias-variance decomposition of MSE gives
$$
    \E[\| A(\hy_{1:n}) - \tA\mu \|_2^2]
    = \| \E[A(\hy_{1:n})] - \tA\mu \|_2^2 + \tr \Var[A(\hy_{1:n})].
$$
Suppose that $\Cov[f(X)] = \hat\Sigma$. Then, the bias and variance terms can be written as follows.
\begin{align*}
    \E [A(\hy_{1:n})] - \tA\mu
    &= \tA \E [y_i] +  \tA \E[\epsilon_i] - \tA\mu
     = \tA \E[\epsilon] \\
    \tr\Var[A(\hy_{1:n})]
    &= \tr(\tA \hat\Sigma \tA^T) / n
\end{align*}
For large enough $n$, we can assume the variance to be negligible. Therefore, we only care about the bias. We can write the bias as follows:
\begin{align*}
    \| \E[A(\hy_{1:n})] - \tA\mu \|_2^2
    &= \| \tA \E[\epsilon] \|_2^2
     = \tr\left( \| \tA \E[\epsilon] \|_2^2 \right) \\
    &= \tr\left( Q^T \E[\epsilon] \E[\epsilon]^T Q \Lambda \right)
     = \sum_{i=1}^d \lambda_i q_i^T \E[\epsilon] \E[\epsilon]^T q_i \\
    &= \sum_{i=1}^d \lambda_i (q_i^T \E[\epsilon])^2
\end{align*}

\chris{This section is still a work in progress.} Therefore, the difference in MSE between Option 1 and Option 2 is as follows. We aim to show that the following quantity is positive:

\begin{align*}
    \frac{1}{m} \sum_{i=1}^d \lambda_i q_i^T \Sigma q_i - \sum_{i=1}^d \lambda_i (q_i^T \E[\epsilon])^2
    &= \sum_{i=1}^d \lambda_i q_i^T \left( \frac{1}{m} \Sigma - \E[\epsilon] \E[\epsilon]^T \right) q_i
\end{align*}

\begin{align*}
    \| \E[A(\hy_{1:n})] - \tA\mu \|_2^2
    &= \tr\left( Q^T \E[\epsilon] \E[\epsilon]^T Q \Lambda \right) \\
    &\leq \tr\left( Q^T \E[\epsilon] \E[\epsilon]^T Q \right) \tr(\Lambda)
     = \tr\left( Q Q^T \E[\epsilon] \E[\epsilon]^T \right) \tr(\Lambda) \\
    &= \tr\left(\E[\epsilon] \E[\epsilon]^T\right) \tr(\Lambda)
     = \left( \sum_{i=1}^d \E[\epsilon_i] \right) \left( \sum_{i=1}^d \lambda_i \right)
\end{align*}

Since we assume $Y \in [0, 1]$, this means that $\epsilon \in [-1, 1]$. From Lemma~\ref{lemma:max}, we know that
$$
    \Pr\left( \E[\epsilon] > \max_i \epsilon_i - 2 (1 - \zeta^{1/m}) \right)
    < \zeta.
$$

We aim to show something like:
$$
    \Pr\left[ \| \mathrm{Bias} \|_2^2 > 3 \| \epsilon \tA \|_2^2 + 3\frac{c^2}{m} \| \tA \mathbf{1} \|_2^2 \right] < \zeta
$$

\subsection{Mean Estimation}
Using the lemmas above, we get the following confidence intervals. For $\zeta \in [0, 1]$, with probability $\geq 1 - 2\zeta$:
$$
    \E[Y] \in \left[
        \frac{1}{n} \sum_{i=1}^n f(X_i) - \epsilon_{(m)} - 2(1-\zeta^{1/m}),
        \frac{1}{n} \sum_{i=1}^n f(X_i) - \epsilon_{(1)} + 2(1-\zeta^{1/m})
    \right]
$$
$$
    \E[Y] \in \left[
        \bar{Y} - \sqrt{-\frac{\ln \zeta}{2m}},
        \bar{Y} + \sqrt{-\frac{\ln \zeta}{2m}}
    \right]
$$



\newpage
\chris{Below this is old}
Now, we will try to show that even if we have 0 error on the $m$ labeled data points, our estimator may still have large bias. Consider a particularly perverse $\epsilon$. Suppose for a subset $\Xc_\mathrm{bad} \subset \Xc$ where $\Pr[\Xc_\mathrm{bad}] = \delta$, we have $\epsilon(x) = \mathbf{1}$, while for all other $x$, $\epsilon(x)=\mathbf{0}$. Then
$$
    \Pr\left[\forall i=1, \dotsc, m.\quad \epsilon(x_i) = \mathbf{0}\right]
    = (1-\delta)^m
    = \zeta > 0
$$
Solving for $\delta$ gives $\delta = 1 - e^{(\ln \zeta)/m} \leq -(\ln \zeta)/m$, using the inequality that $\forall x.\ e^x \geq x + 1$.

\chris{The following claim still doesn't make sense to me. We want to say something like $$\Pr[\E[\epsilon] > b \mid \epsilon_1 = \dotsb = \epsilon_m = \mathbf{0}] = \zeta$$ but how can you properly compute this conditional probability? We don't know $\Pr[\E[\epsilon] > b]$ and we don't know $\Pr[\epsilon_1 = \dotsb = \epsilon_m = \mathbf{0}]$.}
In other words, even when we observe $\epsilon_1, \dotsc, \epsilon_m = \mathbf{0}$, it is still the case that with probability $\zeta$,
$$
    \E[\epsilon] \geq \frac{-\log \zeta}{m} \mathbf{1}
$$
This implies that
\[ \lVert \tA \E[\epsilon] \rVert^2 \geq \left(\frac{-\log \zeta}{m} \right)^2 \mathrm{tr}(\mathrm{1}\mathrm{1}^T \tA \tA^T)  \]

\subsection{Linear Case}\label{sec:linear_case}
We first show the simpler case where $A$ is linear in $y_{1:l}$. For any given set of $x_{1:l}$, for $A$ to be linear in $y_{1:l}$ there must be a sequence of $A_1, A_2, \dotsc, A_l \in \R^{k \times d}$, and $A(y_{1:l}) = \sum_i A_i y_i$. In addition, because it must also be unbiased, so there must be some $\theta$ independent of $l$, such that 
$$
    \theta
    = \E\left[\sum_i A_i y_i\right]
    = \sum_i A_i \E[y_i]
    = \left( \sum_i A_i \right) \mu
$$

\chris{Why is the following claim true?}
This implies that $A_i = \frac{1}{l} \tA(x_i)$. Therefore any such unbiased estimator linear in $y_{1:l}$ must be equal to
$$
    A(x_{1:l}, y_{1:l}) = \frac{1}{l} \sum_i \tA(x_i) y_i
$$
where $\tA: \Xc \to \R^{k \times d}$. Without loss of generality we assume this is how $A$ is defined.


\subsection{Non-linear Case}
Suppose we know that our estimator has asymptotically normal error, which is true for any MLE estimator.
$$
\lim_{l \to \infty} A(y_1, \dotsc, y_l) \to \mathcal{N}(\mu^*, \Sigma/l) $$

The MSE error will be $ \E[(A(y_{1:l}) - \mu^*)^2] $
$$
    \E[(A(y_{1:l}) - \mu^*)^2] = \tr \Sigma / l
$$

% For option 2 we first obtain PAC certificates for the estimation of $y$. Let $e = \E[y - g^*(x)]$, and $e_m = \frac{1}{m} \sum_{i=1}^m (y_i - g^*(x_i))$, then we know by asymptotic normality,  
% \[ e_m \sim \mathcal{N}(e, \Gamma/m) \]

% We need some notion of ``the worst distribution that could typically produce the validation set''

% Note that if $e$ is big, we are already doomed. The only hope is that $e$ is small, and for small $e$ we can use local analysis.
Consider how a small perturbation can affect $A$. Let $\partial_i$ denote the gradient with respect to the $i$-th argument, and let $\epsilon_i = y_i - f(x_i)$. We use a Taylor expansion and get (with notational shorthand of $Y^* = g^*(x_1), \cdots, g^*(x_n)$)
\begin{align*}
    A(y_1, \cdots, y_n) &\approx A(Y^*) + \sum_{i=1}^n \partial_i A(Y^*) \epsilon_i \\
    % &\approx \mathcal{N}(A(g^*(x_1), \cdots, g^*(x_n)), \Gamma)
\end{align*}
The bias of our approach is therefore
$$
    \E [A(y_1, \dotsc, y_n) - A(Y^*)]
    \approx \sum_{i=1}^n \partial_i A(Y^*) \E[\epsilon_i]
$$
Consider a particularly perverse $\epsilon$. Suppose for a subset $\Xc_\mathrm{bad} \subset \Xc$, such that $\Pr[\Xc_\mathrm{bad}] = \delta$, we have $\epsilon(x) = 1$, while for all other $x$, $\epsilon(x)=0$ then we know that
$$
    \Pr[\forall i=1, \dotsc, m.\quad \epsilon(x_i) = 0] = (1-\delta)^m = \zeta
$$
That is we know that $\delta = 1 - e^{(\ln \zeta) / m} \leq -\ln \zeta/m$. Then there is no way to conclude that
$$
    \E [\| A(y_1, \cdots, y_n) - A(Y^*) \|_2^2]
    \leq \frac{-\log \zeta}{m}
$$
% Then we can apply the continuous mapping theorem to conclude that 
% \[ \lVert A(y_1, \cdots, y_n) - A(g^*(x_1), \cdots, g^*(x_n) \rVert \to_D \mathrm{tr}(\mathcal{W}(\Gamma, 1))  \]
% \begin{lemma}
% Let $x_i, i=1, \cdots, n$ be i.i.d. distributed in $\mathbb{R}^d$ with finite covariance, and $A_i, i = 1, \cdots, n \in \mathbb{R}^{m \times d}$. Then 
% \[ \lim_{n \to \infty} \sum_{i} A_i x_i \to_D \mathcal{N}(0, \sum_i A_i \mathrm{Cov}(x_i) A_i^T)\]
% \end{lemma}

For comparison need some method of saying: if $\partial_i A$ is small, then $A$ is stable, and direct estimation should also yield low error.

\section{Appendix}
\subsection{Hoeffding's Inequalities}
If $X_1, \dotsc, X_n \in [a, b]$ are independent random variables, then for any $t > 0$,
\begin{gather}
\Pr[\bar X - \E[X] \geq t] \leq \exp(-2n t^2 / (b-a)^2) \\
\Pr[\bar X - \E[X] \leq -t] \leq \exp(-2n t^2 / (b-a)^2) \\
\Pr\left[\left| \bar X - \E[X] \right| \geq t \right] \leq 2 \exp(-2n t^2 / (b-a)^2)
\end{gather}
In particular,
$$
    \Pr\left( X > \E[X] - t \right)
    \quad=\quad
    1 - \Pr\left( X \leq \E[X] - t \right)
    \quad\geq\quad
    1 - e^{-2 t^2 / (b-a)^2}
$$

\subsection{Cantelli's Inequality}
$$
    \Pr(X > \E[X] - c) \geq 1 - \frac{\sigma^2}{\sigma^2 + c^2}
$$

\subsection{Trace}

\begin{lemma}
Consider two matrices $K, B \in \R^{n \times n}$ where $B$ can be diagonalized as $Q \Lambda Q^T$. Let $q_1, \dotsc, q_n$ be the columns of $Q$, and let $\Lambda = \diag(\lambda_1, \dotsc, \lambda_n)$. Then
$$
    \tr(K B) = \sum_{i=1}^n \lambda_i q_i^T K q_i.
$$
\end{lemma}
\begin{proof}
\begin{align*}
    \tr(KB)
    &= \tr(K Q \Lambda Q^T) \\
    &= \tr(Q^T K Q \Lambda) \\
    &= \sum_{i=1}^n (Q^T K Q)_{ii} \lambda_i \\
    &= \sum_{i=1}^n \lambda_i q_i^T K q_i.
\end{align*}
\end{proof}

\begin{lemma} Let $D = \diag(\bar{d}) \in \R^{n \times n}$ be a diagonal matrix with non-negative entries. For any square matrix $A \in \R^{n \times n}$ with non-negative entries on the diagonal $\bar{a}$,
$$ \tr(A D) \leq \tr(A) \tr(D). $$
The inequality is tight iff $\bar{a}$ and $\bar{d}$ are scalar multiples of each other and each has at most 1 non-zero entry.\footnote{https://math.stackexchange.com/q/853696}
\end{lemma}
\begin{proof}
Let $\bar{a} = (A_{11}, \dotsc, A_{nn})$ denote the diagonal of $A$, and let $\bar{d} = (d_1, \dotsc, d_n)$ denote the diagonal of $D$. Then,
$$ \tr(A D) = \sum_{i=1}^n A_{ii} d_i = \bar{a}^T \bar{d}. $$
Applying the Cauchy-Schwarz Inequality and the fact\footnote{https://math.stackexchange.com/q/245052} that $\forall x.\ \|x\|_2 \leq \|x\|_1$, we have
$$
    | \tr(A D) |
    = | \bar{a}^T \bar{d} |
    \leq \|\bar{a}\|_2 \|\bar{d}\|_2
    \leq \|\bar{a}\|_1 \|\bar{d}\|_1.
$$
The 1st inequality is tight iff $\bar{a}$ and $\bar{d}$ are scalar multiples of each other, and the 2nd inequality is tight iff $\bar{a}$ and $\bar{d}$ each have at most 1 non-zero entry.

If the diagonals of both $A$ and $D$ only have non-negative entries, then
$$
    \bar{a}^T \bar{d} > 0,
    \qquad
    \|\bar{a}\|_1 = \tr(A),
    \qquad\text{and}\qquad
    \|\bar{d}\|_1 = tr(D).
$$
Therefore, $\tr(AD) \leq \tr(A) \tr(D)$.
\end{proof}

\section{Related Work}

Semi-supervised domain adaptation, especially few shot, one shot

Semi-supervised learning

\verb|https://docs.google.com/document/d/1sVsXDsRtx-tJAz_sJ3YLV7iaYKHcTlFgqQZVnUPeMbI/edit?usp=sharing|

\section{Experiments}

